SAT-based Formal Fault-Resistance Verification of Cryptographic Circuits

Fault injection attacks represent a type of active, physical attack against cryptographic circuits. Various countermeasures have been proposed to thwart such attacks, the design and implementation of which are, however, intricate, error-prone, and laborious. The current formal fault-resistance verification approaches are limited in efficiency and scalability. In this paper, we formalize the fault-resistance verification problem which is shown to be NP-complete. We then devise a novel approach for encoding the fault-resistance verification problem as the Boolean satisfiability (SAT) problem so that off-the-shelf SAT solvers can be utilized. The approach is implemented in an open-source tool FIRMER which is evaluated extensively on realistic cryptographic circuit benchmarks. The experimental results show that FIRMER is able to verify fault-resistance of almost all (46/48) benchmarks in 3 minutes (the other two are verified in 35 minutes). In contrast, the prior approach fails on 23 fault-resistance verification tasks even after 24 hours (per task).

==> sections/optimization.tex <==
%\section{Acceleration Techniques for Fault-resistance Verification}
%\label{chap:optimization}



\begin{comment}
\subsection{Proposition and Proof}
With the basic SAT-based verification in place, we performed further optimization. We present our optimization in the following three propositions.

\begin{table}[]
\caption{The output of the gate after injecting various types of faults}
\label{table1}
\centering
\begin{tabular}{|c|c|c|}
\toprule
fault type &    &    \\
\midrule
$g^o$ & 0 & 1 \\
$g^o_{bf}$ & 1 & 0 \\
$g^o_{s}$ & 0 & 0 \\
$g^o_{r}$ & 1 & 1 \\
\bottomrule
\end{tabular}
\end{table}


\begin{proposition}
    If the circuit is secure when injecting fault $\tau_{bf}$, it is also secure when injecting fault $\tau_{s}$, $\tau_{r}$ and $\tau_{sr}$.
\end{proposition}




% \begin{lemma}
% If the circuit is safe when inject fault $\tau_{bf}$, it is also safe when inject fault $\tau_{s}$, $\tau_{r}$ and $\tau_{sr}$.
% \label{lem-1}
% \end{lemma}

\begin{proof}
Suppose the output of a gate is $g^o$. For a gate without fault, suppose the value of the output is $g^o=\{ 0, 1\}$. If the fault is $\tau_{bf}$, then the value of the output is $g^o_{bf}=\{ 1, 0\}$. If the fault is $\tau_{set}$, then the output is $g^o_{set}=\{ 1, 1\}$. If the fault is $\tau_{reset}$, then the output is $g^o_{reset}=\{ 0, 0\}$. The outputs of all gates injected with faults are shown in \cref{table1}. Thus we can conclude that: if the output of gate is 0, inject $\tau_{bf}$ will same with inject $\tau_{r}$, and inject $\tau_{s}$ will not change the result. If the output of gate is 1, inject $\tau_{bf}$ will same with inject $\tau_{s}$, and inject $\tau_{r}$ will not change the result. This means that the bit flip contains the other two fault types. So if $\tau_{bf}$ is secure, $\tau_{s}$, $\tau_{r}$ and $\tau_{sr}$ also secure.
\end{proof}

According Proposition 4.1, the subfomula $\Psi_{enc}$ is then simplified as $\Psi_{enc}^{simp} = (\bigwedge_{i=1}^q(p_{out}^i=c_{gi}?(p_{in1}^i\ \tau_{bf}\ p_{in2}^i):(p_{in1}^i\ p_{op}^i\ p_{in2}^i)))$, where $\tau$ is replaced by $\tau_{bf}$.


% \begin{proposition}
%     If the circuit is secure with fault model $\zeta (n,t,l)$, it is also secure with fault model $\zeta (n-1, t, l)$.
% \end{proposition}

% \begin{lemma}
% If the circuit is safe with fault model $\zeta (n,t,l)$, it is also safe with fault model $\zeta (n-1, t, l)$.
% \label{lem-1}
% \end{lemma}
%  \begin{proof}
% Suppose there is a circuit $\mathbf{C}$ that under fault model $\zeta (n,t,l)$ is safe but under fault model $\zeta (n-1, t, l)$ is not secure. Define the set of fault injection gates in $\mathbf{C}$ under $\zeta (n, t, l)$ as $\mathcal{G}_{fault}^{n}$. Next we construct a gate $g_{new}$ that is independent of the output. Then $g_{new}$ and $\mathbf{C}$ form a new circuit $\mathbf{C}'$. Now we inject faults in $\mathbf{C}'$. We select $n-1$ gates in $\mathcal{G}_{fault}^{n-1}$ of $\mathbf{C}$ and the new gate $g_{new}$. Since the new gate does not affect the output, $\mathbf{C}'$ under $\zeta (n, t, l)$ is still not secure cause $\mathbf{C}$ under $\zeta (n-1, t, l)$ is not secure. It contradicts the hypothesis. So the theorem is proved.
% \end{proof}

% According to proposition 3, we can further simplify the subformula $\Psi_{v}\wedge\Psi_{n}$ as $\Psi_{v}^{simp}\wedge\Psi_{n}^{simp} = ((\sum_{i=0}^{x} c_{ci} = v) \wedge (\sum_{j=0}^{y} c_{gj} = n))$.

% \begin{lemma}
% Define a gate $g$'s successor to be the gate connected to the $g$'s output. If a gate has only one direct successor, injecting a fault at this gate is equivalent to injecting a fault at its direct successor.
% \label{lem-1}
% \end{lemma}


\begin{proposition}
    Define a gate $g$'s successor to be the gate connected to the $g$'s output. If a gate has only one direct successor, injecting a fault at this gate is equivalent to injecting a fault at its direct successor.
\end{proposition}

\begin{proof}
Suppose a injected fault gate $g^{fault}$. Consider it has only one direct successor $g_{s}$. Considering fault propagation, since it has only one direct successor, the fault will have only one propagation path until the next gate. Therefore, injecting faults at either of these two gates is equivalent.
\end{proof}

According to Proposition 4.2, we present the optimization results on RECTANGLE S-box. Fig \ref{fig:optimize circuit} shows the detail.
 In this circuit, gates $s1, s4, s5, s7, s8, p1, p2, p3, p4, p5$ are only used once. Thus, inject fault into those gates are similar with inject fault into their successor. Hence, we reduced the number of gates that need to be injected from 18 to 8.

 Based on the above optimization, the formula $\Phi$ in Equation \ref{encoding phi} can be further simplified to $\Phi_{simp}$ as  shown in Equation \ref{optimization phi}.

\begin{figure}[tbp]
    \centering
    \includegraphics[width=1\linewidth]{figs/optimize_circuit.pdf}
    \caption{The RECTANGLE S-box implementation circuit with static analysis optimization.}
    \label{fig:optimize circuit}
\end{figure}

\begin{equation}
\label{optimization phi}
\Phi_{simp}=
\left(
\begin{array}{lll}
s1 &= b \oplus c &\wedge\\
s2 &= c_{g1}\ ?\ (\tau\ c):(\neg c)&\wedge\\
s3 &= c_{g2}\ ?\ (b\ \tau\ a):(b \oplus a)&\wedge\\
s4 &= s2 \wedge d&\wedge\\
s5 &= s2 \vee a &\wedge\\
z  &= c_{g3}\ ?\ (s3\ \tau\ s4):(s3 \oplus s4)&\wedge\\
s6 &= c_{g4}\ ?\ (s5\ \tau\ d):(s5 \oplus d) &\wedge\\
s7 &= s3 \wedge s6&\wedge\\
s8 &= s1 \vee z&\wedge\\
w  &= c_{g5}\ ?\ (s1\ \tau\ s7):(s1 \oplus s7)&\wedge\\
x  &= c_{g6}\ ?\ (s8\ \tau\ s6):(s8 \oplus s6)&\wedge\\
y  &= c_{g7}\ ?\ (b\ \tau\ s6):(b \oplus s6)\wedge\\
p1 &= (c\ \overline{\oplus}\ d)&\wedge\\
p2 &= (c\vee a)&\wedge\\
p3 &= (a \wedge p1)&\wedge\\
p4 &= (d\ \overline{\wedge}\ p2)&\wedge\\
p5 &= (b \wedge p4)&\wedge\\
p6 &= c_{g8}\ ?\ (p3\ \tau\ p5):(p3 \vee p5)
\end{array} \right)
\wedge (\sum_{i=1}^{8}c_{gi}\le n) \wedge (((\bigwedge_{out=w}^z(out\oplus out'))\wedge(\neg\ flag))=0)
\end{equation}


We give the algorithm of proposition 3 and the final algorithm for verification based on the above optimization in Section \ref{algorithm}.


\subsection{Algorithm}
\label{algorithm}

We first give the algorithm for proposition 3.

Algorithm \ref{static analysis} introduce the optimization of static analysis. Given a abstract model $\mathcal{D}$ for digital circuit $\mathbf{C}$, we iteratively access each tuple. For each tuple $n$, if its type is in binary operation $O_b$, then it must has two input, which means $n$ is a direct successor to these two inputs. So we add it into the successor set $\mathbf{s}_{n_{in1}}$ and $\mathbf{s}_{n_{in2}}$. If the type is in unary operation, we add it into $\mathbf{s}_{n_{in1}}$ cause unary operation only has one input. Line 3-10 is the detailed algorithm. After that, we select the gate to inject fault. For gate $g_i$, if its size of successor set $\mathbf{s}_{g_{i}}$ equal to 1, we ignore it. If the size is greater than 1, we inject fault in this gate.



\begin{algorithm}
\SetAlgoLined
\caption{Static Analysis}
\label{static analysis}
  \KwIn{Synchronous circuit $\mathcal{S}$ and blacklist $\mathbf{B}$ .}
  \KwOut{Set of gates with successors greater than one.}
  Define $q$ as the queue\;
  Define the set of successors of a gate as $\mathbf{s}$\;
  Define $\mathcal{SU}$ as the set of gates with successors greater than one\;
  \For{tuple $p$ in $\mathcal{S}$}{
    \eIf{$p_{type} \in O_u$}{
        $g_i\gets p_{index}$, $g_j\gets p_{input}$\;
        $\mathbf{s}_{g_j}\gets \mathbf{s}_{g_j} \cup \mathbf{s}_{g_i}$\;
    }{
        $g_i\gets p_{index}$, $g_j\gets p_{input1}$, $g_k\gets p_{input2}$\;
        $\mathbf{s}_{g_j}\gets \mathbf{s}_{g_j} \cup \mathbf{s}_{g_i}$\;
        $\mathbf{s}_{g_k}\gets \mathbf{s}_{g_k} \cup \mathbf{s}_{g_i}$\;
    }
  }
    \For{tuple $p$ in $\mathcal{S}$} {
        $g_i\gets p_{index}$\;
        \uIf {($\mathbf{s}_{g_i}>1$) or ($\exists s\in \mathbf{s}_{g_i}$,$p_{type}^s=out$ or $s\in $blacklist)}{
            $\mathcal{SU} = \mathcal{SU} \wedge g_i$\;
        }
    }
\Return{ $\mathcal{S}$ }
\end{algorithm}

% \begin{algorithm}
% \caption{Static Analysis}
% \label{static analysis}
% \hspace*{0.02in} {\bf Input:}
% Abstract model $\mathcal{D}$.\\
% \hspace*{0.02in} {\bf Output:}
% Set of gates with successors greater than one.
%   \begin{algorithmic}[1]
%     \State Define the set of successors of a gate as $\mathbf{s}$.
%     \State Define $\mathcal{S}$ as the set of gates with successors greater than one.
%     \For {tuple $p$ in $\mathcal{D}$}
%         \If {$p_{type}$ = output or $p_{type} \in O_u$}
%             \State $g_i\gets p_{index}$, $g_j\gets p_{input}$
%             \State $\mathbf{s}_{g_j}\gets \mathbf{s}_{g_j} \cup \mathbf{s}_{g_i}$
%         \EndIf
%         \If {$p_{type} \in O_b$}
%             \State $g_i\gets p_{index}$, $g_j\gets p_{input1}$, $g_k\gets p_{input2}$
%             \State $\mathbf{s}_{g_j}\gets \mathbf{s}_{g_j} \cup \mathbf{s}_{g_i}$
%             \State $\mathbf{s}_{g_k}\gets \mathbf{s}_{g_k} \cup \mathbf{s}_{g_i}$
%         \EndIf
%     \EndFor
%     \For{tuple $p$ in $\mathcal{D}$}
%         \State $g_i\gets p_{index}$
%         \If {$\mathbf{s}_{g_i}==1$}
%             \State continue
%         \Else
%             \State $\mathcal{S} = \mathcal{S} \wedge g_i$
%         \EndIf
%     \EndFor
%     \State return $\mathcal{S}$
%   \end{algorithmic}
% \end{algorithm}



\begin{algorithm}
\SetAlgoLined
\caption{Verfication}
\label{Verifcation}
  \KwIn{Abstract model $\mathcal{D}$, fault model $\zeta (n_e,n_c, \tau_{bf}, l)$, number of variate $v$.}
  \KwOut{UNSATISFIABLE or SATISFIABLE.}
  $\mathcal{S} =$ Static analysis($\mathcal{D}$)\;
  Encoding the abstract model into $\Phi_{simp}$\;
  Solve $\Phi_{simp}$ by SAT solver\;
    \eIf {$\Phi_{simp}$ is UNSATISFIABLE}
        {\Return{The circuit is security}}
        {\Return{The circuit is not security}}
\end{algorithm}

Next we give the overall algorithm of out verification in Algorithm \ref{Verifcation}. The input of the algorithm is the abstract model $\mathcal{D}$ and the fault model $\zeta(\Nn_e,\Nn_c,\mathcal{T},\CR)$, where $\mathcal{T}$is $\tau_{bf}$. First, we do static analysis on the model. Then we encode the model into  the simplified formula $\Phi_{simp}$. After we get the formula $\Phi_{simp}$, we give it to SAT solver. The result is UNSATISFIABLE or SATISFIABLE. If the result is UNSATISFIABLE, the circuit is security. If the result is SATISFIABLE, the circuit is not security.
\end{comment}


==> sections/outline.tex <==
- 1. Intro
- 2. Preliminary
    - background / problem
    - Circuit model
        - 整体先描述一下circuit
        - Formall
        - logic stage
        - example
    - Fault Injection Attack
        - what
        - how
        - result
        - Formally, model
    - Countermeasures
        - detection
        - correction
        - example
    - Security
        - Definition \begin{definition} xxx \end{definition}
        - Given a fault model ..., iff
- 3. SAT-based Approach
    - Encoding: Given a cirit, \psi (参考宋老师发的文章的定义
        - circuit
        - choose location + assign a operation
        - security check
        - connect with "and"
        - propsition: iff \psi
        - example: 前面的circuit，用\psi 表示出来
    - Algo if \psi = sat ... else ...
- 4. Optimization
    - Lemma 1 only bit-flip can cover mixed fault
        - formal definition
        - proof
        - example: bf，公式化简\psi
    - Lemma 2 n - n-1
        -
        -
    - Lemma 3 static
        -
        -
        - example: 跳出来只用了一次，\psi
        - algo
    - Optimization Algo (overall algo)
        - circuit
        - use lemma1
        - use lemma2
        - use lemma3
        - \psi
        - if ...
- 5. Exp
- 6. Related
- 7. Conclusion
